New Confidence Measures for Statistical Machine Translation

A confidence measure is able to estimate the reliability of an hypothesis provided by a machine translation system. The problem of confidence measure can be seen as a process of testing : we want to decide whether the most probable sequence of words provided by the machine translation system is correct or not. In the following we describe several original word-level confidence measures for machine translation, based on mutual information, n-gram language model and lexical features language model. We evaluate how well they perform individually or together, and show that using a combination of confidence measures based on mutual information yields a classification error rate as low as 25.1% with an F-measure of 0.708.

==> abstract.tex <==
% \fontsize{9}{11}\selectfont In the following we describe several original word-level confidence measures for machine translation, based on mutual information, n-gram language model and lexical features language model. We evaluate how well they perform individually or together.
% The abstract should summarize the
% contents of the paper and should contain at least 70 and at most 200
% words. The text should be set in 9-point font size.

\fontsize{9}{11}\selectfont A confidence measure is able to estimate the reliability of an hypothesis provided by a machine translation system.
The problem of confidence measure can be seen as a process of testing : we want to decide whether the most probable sequence of words provided by the machine translation system is correct or not.
In the following we describe several original word-level confidence measures for machine translation, based
on mutual information, n-gram language model and lexical features language model. We evaluate how well
they perform individually or together, and show that using a combination of confidence measures based on mutual information yields a classification error rate as low as 25.1\% with an F-measure of 0.708.


==> authors.tex <==
\author{{\textmd {\textbf }}\\
  \fontsize{11}{13}\selectfont
  Sylvain Raybaud, Caroline Lavecchia, David Langlois, Kamel Sma\"ili\\
  \fontsize{9}{11}\selectfont
  \textit{PAROLE team, LORIA, Campus Scientifique, BP 239, 54506 Vandoeuvre-lès-Nancy FRANCE}\\
  \fontsize{9}{11}\selectfont
  \textit{\{raybauds,lavecchi,langlois,smaili\}@loria.fr}\\[12pt]
  %
%   \fontsize{11}{13}\selectfont
%   Third Author Name\\
%   \fontsize{9}{11}\selectfont
%   \textit{Department of Computing, Main University, MySecondTown, MyCountry}\\
%   \fontsize{9}{11}\selectfont
%   \textit{t\_author@xy.mu.edu}\\[12pt]
  %
  % repeat previous group of commands here for further authors
}


==> keywords.tex <==
\fontsize{9}{11}\selectfont confidence measure, statistical machine translation, mutual information, linguistic features language model, n-gram language model
% The paper should have at least one
% keyword. The text should be set in 9-point font size and without the
% use of bold or italic font style.


==> title.tex <==
% The Title is all in Uppercase
% \newcommand{\mytitle}{\uppercase{Authors' Instructions}\\
% % The Subtitle should have initial letters capitalized
% \fontsize{13}{15}\selectfont \textit{Preparation of Camera-Ready
% Contributions to INSTICC Proceedings}
% }

\newcommand{\mytitle}{\uppercase{New confidence measures for statistical machine translation}\\
% The Subtitle should have initial letters capitalized
% \fontsize{13}{15}\selectfont \textit{On the Use of Triggers and Target Language Model for Word-Level Confidence Estimation}
\fontsize{13}{15}\selectfont \textit{}
}

